An Empirical Survey on Co-simulation: Promising Standards, Challenges and Research Needs

Co-simulation is a promising approach for the modelling and simulation of complex systems, that makes use of mature simulation tools in the respective domains. It has been applied in wildly different domains, oftentimes without a comprehensive study of the impact to the simulation results. As a consequence, over the recent years, researchers have set out to understand the essential challenges arising from the application of this technique. This paper complements the existing surveys in that the social and empirical aspects were addressed. More than 50 experts participated in a two-stage Delphi study to determine current challenges, research needs and promising standards and tools. Furthermore, an analysis of the strengths, weakness, opportunities and threats of co-simulation utilizing the analytic hierarchy process resulting in a SWOT-AHP analysis is presented. The empirical results of this study show that experts consider the FMI standard to be the most promising standard for continuous time, discrete event and hybrid co-simulation. The results of the SWOT-AHP analysis indicate that factors related to strengths and opportunities predominate.

==> commands.tex <==
% Flag that controls the display of comments.
\newif\ifcomments
% Enable/Disable comments.
\commentstrue % Comment to disable

\newcommand{\claudio}[1]{%
\ifcomments %
\textbf{\textcolor{red}{\scriptsize Claudio: #1}} %
\else %
 %
\fi%
}%

\newcommand{\gerald}[1]{%
\ifcomments %
\textbf{\textcolor{blue}{\scriptsize Gerald: #1}} %
\else %
 %
\fi%
}%

\newcommand{\sepp}[1]{%
\ifcomments %
\textbf{\textcolor{green}{\scriptsize Sepp: #1}} %
\else %
 %
\fi%
}%

\newcommand{\georg}[1]{%
\ifcomments %
\textbf{\textcolor{orange}{\scriptsize Georg: #1}} %
\else %
 %
\fi%
}%

\newcommand{\irene}[1]{%
\ifcomments %
\textbf{\textcolor{black}{\scriptsize Irene: #1}} %
\else %
 %
\fi%
}%

\newcommand{\alfred}[1]{%
\ifcomments %
\textbf{\textcolor{red}{\scriptsize Alfred: #1}} %
\else %
 %
\fi%
}%

\newcommand{\thierry}[1]{%
\ifcomments %
\textbf{\textcolor{green}{\scriptsize Thierry: #1}} %
\else %
 %
\fi%
}%


\newcommand{\footurl}[1]{\footnote{\url{#1}}}


